Programming Complex Systems

Classical programming languages cannot model essential elements of complex systems such as true random number generation. This paper develops a formal programming language called the lambda-q calculus that addresses the fundamental properties of complex systems. This formal language allows the expression of quantumized algorithms, which are extensions of randomized algorithms in that probabilities can be negative, and events can cancel out. An illustration of the power of quantumized algorithms is the ability to efficiently solve the satisfiability problem, something that many believe is beyond the capability of classical computers. This paper proves that the lambda-q calculus is not only capable of solving satisfiability but can also simulate such complex systems as quantum computers. Since satisfiability is believed to be beyond the capabilities of quantum computers, the lambda-q calculus may be strictly stronger.

==> ICCSsty.tex <==
% -*- Mode:TeX -*-
% iccssty.tex (LATEX style for International Conference on Complex Systems); LaTeX2e only!
% email to yaneer@necsi.org for questions

 \makeatletter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  OVERALL GEOMETRY (text height and width, two-column, etc.)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We want to cram as much information as possible onto a page, using
% two columns and rather narrow margins. Intended to be used at 10pt.
%
% To simplify interfacing with PostScript figures, we use TeX's BIG POINT
% (bp = 1/72in), which is identical to the PostScript default unit,
% rather than Tex's POINT (pt = 1/72.27in).

% ======== PAGE SIZE AND STYLE ========
% A typical laser printer will not put ink all the way to the edge of the page
% (bleeding), but will leave from 1/8" to 1/4" of virgin edge. For reference,
%	1    in	= 72 bp
%	1/2  in	= 36 bp
%	3/8  in	= 27 bp
%	1/3  in	= 24 bp
%	1/4  in = 18 bp
%	1/8  in =  9 bp
%	1/16 in =  4.5 bp

% -------- Vertical --------
 \pagestyle{plain}	% Page number will always go in the footer
 \headheight	0bp	% No header. These two parameters had been set by
 \headsep	0bp	% \pagestyle, but we reset them to zero.
 \footskip	27bp	% We also reset this to 3/8".
 \topmargin	-0.25in	% We want 3/4" top and bottom margins, plus 3/8" footer;
 \textheight	9.125in	% that leaves 11"-15/8" = 9"+1/8" for the text.

% -------- Horizontal --------
			% two columns of 248 bp, separated by 12bp
 \textwidth	508bp	% 7in + 4bp
 \oddsidemargin -20bp	% that leaves 52bp, ie 3/4in - 2bp
 \evensidemargin-20bp
 \columnsep=12bp	% default (@ 10bp) is 10bp; column is 254bp-6bp=248bp
 \normalmarginpar
% with -20bp of sidemargin, we have  52bp of margin, to be used as follows
 \marginparwidth 36bp	%  8/16"
 \marginparsep   4bp	%  a little less than 1/16''
% virgin edge	12bp

% column width is 248 bp

 \def\BOOKLET{		% This is only for very compact proofing at 5.5x8.5
 \topmargin	-0.50in	% We want 1/2" top and bottom margins, plus 3/8" footer;
 \textheight=865bp % for ps.quad output
 \footskip	18bp	% We also reset this to 3/8".
 \columnsep=8bp
 \textwidth	522bp	% 7in + 4bp
 \oddsidemargin -27bp	% that leaves 5/4in total between left and rite
			% which dvips may do 3/4 inside and 1/2 outside
 \evensidemargin-27bp
% \columnseprule.2pt
}

 \def\BOOK{		% This is for ordinary proofing in lettersize
 \topmargin	-0.50in	% We want 1/2" top and bottom margins, plus 3/8" footer;
 \textheight	9.75in
 \footskip	27bp	% We also reset this to 3/8".
 \columnsep	10bp
 \textwidth	7.25in	% 7in + 4bp
 \@twosidetrue
% \oddsidemargin -27bp	% that leaves 5/4in total between left and rite
			% which dvips may do 3/4 inside and 1/2 outside
% \evensidemargin-27bp
% \oddsidemargin -27bp	% that leaves 5/4in total between left and rite
			% which dvips may do 3/4 inside and 1/2 outside
 \oddsidemargin -19bp
 \evensidemargin-35bp
}

%\BOOKLET
\BOOK

% ======== TWO_COLUMN STUFF ========
\twocolumn
\sloppy
\flushbottom
\parindent 1em
\leftmargini 2em
\leftmarginv .5em
\leftmarginvi .5em

% \linewidth	is the current line width (a column in twocolumn style,
%		width of text in a parbox, etc.)
% \columnsep	is the separation between the two columns
% \columnwidth	is the column width, = (\textwidth-\columnsep)/2


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  TITLE SECTION (TITLE, AUTHOR, ETC.)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The title banner will be flushright. The left 3/10 of the title banner
% is reserved for a ``proofbox'' with editorial information.
%
% ---------------------------------------------------------------
% | [proofbox here]	|				  TITLE |
% |			|				 Author |
% |			|	        Affiliation and address |
% ---------------------------------------------------------------
% | left column			| right column			|
% | ...				| ...				|

\def\Mail#1 #2 {\gdef\thecontact{#1}\gdef\theaddr{#2}}
\def\Range#1 #2 {\gdef\thefirstpage{#1}\gdef\thelastpage{#2}}
{\let\'\mail \expandafter\Mail\' }	% do not remove space between ' and }
{\let\'\prange \expandafter\Range\' }	% do not remove space between ' and }
 \setcounter{page}{\thefirstpage}
 \gdef\@proofbox{\relax}
 \long\def\proofbox#1{\gdef\@proofbox{#1}}
 \long\def\timestamp{}
 \proofbox{\sloppy\small Proceedings of the %
% \hfill\setbox0=\hbox{\lower3ex\hbox{\includegraphics[scale=.30]{Psi96.ps}}}\ht0=0pt\dp0=0pt\\{\bf International Conference\\ on Complex Systems}\\
\hfill\ht0=0pt\dp0=0pt\\{\bf International Conference\\ on Complex Systems}\\
Nashua, NH, 21--26 Sept.\ 1997.\par
 \medskip
 Y. Bar-Yam
(ed.), New England Complex Systems Institute (1997)
\ifnum\thefirstpage=\thelastpage\thefirstpage\else\thefirstpage--\thelastpage\fi
.\par Also on-line in the {\sl InterJournal}.%
 \ifx\timestamp\@empty\else\par\medskip\timestamp\fi}

 \def\affil#1{\\{\small#1\par}}
 \gdef\@author{John Doe1\affil{No-Name University, Shipping Dept.}}
 \long\def\author#1{\gdef\@author{#1}}

 \gdef\@abstract{}
 \long\def\abstract#1{\gdef\@abstract{#1}}


\def\@maketitle{\newpage\leavevmode
  \begin{minipage}[t]{0.32\textwidth}
    \hrule height0pt
%    \raggedright
    \mbox{}\par
    \@proofbox
  \end{minipage}\hfil
  \begin{minipage}[t]{0.68\textwidth}
    \hrule height0pt
    \raggedleft
    \LARGE\@title\par
    \vskip4pt
    \large\@author
  \end{minipage}
  \vskip8pt
  \ifx\@abstract\@empty\else{\vskip.5em\leftskip1.25in\parskip4pt\small\@abstract\par\vskip.5em}\fi
  \rule{\textwidth}{0.4pt}
  \vskip16pt}

\let\trm\textrm
\let\tbf\textbf
\let\tsl\textsl
\let\ttt\texttt
\let\tsc\textsc

 \sloppy


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  TITLE SECTION (TITLE, AUTHOR, ETC.)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 %======================== EMPHASIS ========================
 %% Use boldface for terms being defined
 \let\tdf\textbf
 \let\df\bf

 %% Use slanted rather than italic for emphasis
\DeclareRobustCommand\em
        {\@nomath\em \ifdim \fontdimen\@ne\font >\z@
                       \upshape \else \slshape \fi}
\let\tem\emph

 %%	use \sl rather than \it in theorems [to be upgraded]
\def\@begintheorem#1#2{\sl \trivlist \item[\hskip \labelsep{\bf #1\ #2}]}
\def\@opargbegintheorem#1#2#3{\sl \trivlist
     \item[\hskip \labelsep{\bf #1\ #2\ (#3)}]}

 %======================== CROSS-REFERENCING ==================
 \newcommand{\sect}[1]{\S\ref{sect:#1}}      % Ref. to section or subsection
                                        %   to appear as, say, $2.37
 \newcommand{\baresect}[1]{\ref{sect:#1}}      % Ref. to one more section or
                                 %    subsection to appear as, say, 2.37
 \newcommand{\eq}[1]{(\ref{eq:#1})}	% Ref. to equation
                                        %   to appear as, say, (2.37)
 \newcommand{\foot}[1]{footnote \ref{foot:#1}} % Ref. to footnote
                                        %   to appear as, say, `footnote 7'.
 \newcommand{\fig}[1]{Fig.~\ref{fig:#1}}

 \newcommand{\sectlabel}[1]{\label{sect:#1}}
 \newcommand{\eqlabel}[1]{\label{eq:#1}}
 \newcommand{\figlabel}[1]{\label{fig:#1}}

 %======================== SECTIONING ========================
 %% Small sections
% \newcommand{\smallsection}[1]{\par\medskip\noindent{\em#1}\par\smallskip}
 \let\smallsection\subsubsection \setcounter{secnumdepth}{2}
 \newcommand{\parhead}[1]{\tsl{#1}.\quad} % Distinguished paragraph
		% heading; slanted, followed by \quad

 %% allow printing 0 as a section (or subsection, item, etc.) number
% \def\@arabic#1{\ifnum #1>0 \number #1\fi} % original definition
  \def\@arabic#1{\number #1} % my redefinition

 %======================== FIGURES ========================
 %% change captions from \normalsize to \small
\long\def\@makecaption#1#2{
	\vskip\abovecaptionskip
	\sbox\@tempboxa{{\small #1: #2}}%
	\ifdim\wd\@tempboxa>\hsize
	    {\small #1: #2\par}
	\else
	   \global\@minipagefalse
	   \hbox to\hsize{\hfil\box\@tempboxa\hfil}
	\fi
	\vskip \belowcaptionskip}

\def\figstrut#1{\hbox to\linewidth{\vrule height#1\hfill}}

%%%% Single-column figure
\newcommand{\Fig}[4][!htb]{% [position] label, picture, caption
\begin{figure}[#1]
 \centering\leavevmode#3%
 \caption{#4}
 \figlabel{#2}
\end{figure}                 }
 \let\figonecol\Fig

%%%% Two-column figure
 \newcommand{\Figwide}[4][!t]{% [position] label, picture, caption
 \begin{figure*}[#1]
  \centering\leavevmode#3%
  \caption{#4}
 \figlabel{#2}
 \end{figure*}                 }
 \let\figtwocol\Figwide

%%%% Float-page figure
 \newcommand{\Figpage}[3]{% label, picture, caption
 \begin{figure*}[p] 
  \centering\leavevmode#2%
  \caption{#3}
 \figlabel{#1}
 \end{figure*}                 }
 \let\figpage\Figpage

% ========= VERBATIMS ========

%\comp is like \verb, but inserts a thin space before and after text

\def\comppad{\thinspace}
\def\comp{\comppad\begingroup \tt \let\do\@makeother \dospecials 
          \@ifstar{\@scomp}{\@comp}}
\def\@scomp#1{\def\@tempa ##1#1{##1\endgroup\comppad}\@tempa}
\def\@comp{\obeyspaces \frenchspacing \@scomp}

%****************************************************************

\def\qed{\vrule height1.2ex width1ex depth.1ex}
\newenvironment{proof}{\par\noindent{\sc Proof}\quad}{\qed\par\smallskip}

\makeatother
\endinput


